Advancing Environmental Sustainability in Data Centers via Carbon Depreciation Models

Recent improvements in energy efficiency and renewable energy integration have increased the relative importance of embodied carbon in data centers, motivating improved provisioning strategies. Conventional approaches primarily minimize operational energy, but this perspective is increasingly insufficient for sustainability. In this paper, we propose carbon depreciation models to encourage longer hardware lifetimes. Carbon depreciation assigns a larger portion of embodied carbon to newly provisioned servers, discouraging unnecessary deployment of new hardware. As a result, new servers are provisioned mainly for jobs with strict quality-of-service (QoS) constraints, while older servers, whose embodied carbon has largely been recovered, are used for other workloads. We further argue that both embodied carbon and operational carbon from server idle time should be recovered during active jobs, encouraging provisioning strategies that maintain high utilization. We show that prior carbon accounting strategies can be counterproductive: under a greedy scheduler minimizing carbon under QoS constraints, jobs are priced as 25% cheaper on new hardware than on older hardware. In contrast, our approach uses a greedy scheduler that prioritizes older hardware through non-linear carbon depreciation, promoting sustainable provisioning. Experimental results show carbon reductions of 28-57%, depending on server lifetime assumptions.

==> contents/5.5_Notes_of_Flow.tex <==
\section{Notes on Flow of Paper}

\akj{Motivation: Carbon and \$ cost for a data center or aligned but not identical}

\akj{$C_{op}$ is decreasing with renewable integration.  Over generation can make this $\approx 0$.  $C_{emb}$ is increasing, but more importantly has limits of how much it can be reduced.  Even with full renewable integration, semiconductors require 30--45\% of their current carbon equivalent during fabrication.}

\akj{Electricity costs \$, systems cost \$, system costs may be falling, energy costs will remain substantial for renewable energy.}

\akj{Thus, carbon optimization must target primarily $C_{emb}$ while \$ optimization remains a function of op and sys costs.}

\akj{Discuss how $C_{emb}$ must all be recovered.  It is insufficient to just consider the $\delta$ of your particular job, it must also consider the load of that machine.}
\ppz{For example, running the same task on an idling data center should cost more than on a busy data center.}

\akj{Provisioning data centers have realized that they need to keep systems in place for longer lifetimes.}

\akj{Discuss how linear job costs is impractical because it prefers the fastest available hardware.  If $C_{job} = C_{emb}*\delta_{t}/L+C_{op}*\delta_{t}$ what happens?  If $C_{emb}\approx C_{emb}'$ and $\delta_{t} > \delta_{t}'$ AND $C_{op} > C_{op}'$ then we much prefer system' (newer system).  So newer system gets heavily loaded, older systems are underutilized, the provisioning is encouraged to get more new systems.}
\ppz{data here}

\akj{we need a way for jobs to prefer using the older system.  As long as the older system can meet QoS, it should have a sustainability advantage.  To accomplish this, $C_{emb}$ cannot be linearly distributed across the lifetime.  $C_{emb}$ should be more heavily recouped in year 1 versus later years.  Now, if $C_{op} \approx 0$ (or is approaching 0) due to heavy renewable integration, then $C_{emb}$ dominates.  Now $C_{emb} << C_{emb}'$.  Thus $C_{job} = C_{emb}*model_{dep}+C_{op}*\delta_{t} \rightarrow$ a function of the $C_{emb}$, which will prefer the older system.}
\ppz{data here}

\akj{two knobs: 1 is cost of the job ($model_{dep}$), and 1 is dealing with the idle.  One methodology could be to go with the traditional idea, which is user only pays for the job.  Then we need to show that the jobs are expensive on the wrong resource. }
\ppz{This is to say that using the traditional model (not considering idle time), we keep older machines in service, so our model should favor them for jobs.\\
00: linear, not considering idle leads to faster machine;\\
10: linear, considering idle leads to consider utilization;\\
01: ddb, not considering idle time leads to scheduling on the older machine;\\
11: ddb, considering idle time leads to a preference towards the older machine, also consider utilization match.\\
}
\akj{If we go with the new approach, which is all the $C_{emb}$ must be applied, you have to pay for idle time, this will push the provisioning to be closely tuned to the need.  (This has a problem, which is how to deal with burstiness).  }

\akj{If we include idle time into $\delta$ ($\delta = \delta_j+\delta_{idle}$) this will further penalize underutilized newer machines.  This is impactful for $C_{emb}$ and $C_{op}$ (unless the latter is near 0).}

\akj{This is cool-tax, or high performance tax :D}
\ppz{This is cool-tax, or high performance carbon cost. In dollar cost, the new machine is 1.5x faster but costs 10x more.}

\akj{This allows greedy user carbon optimization to lead to better provisioning strategies as they are now aligned.  In fact, the goal here is to have data center utilization $\approx$ 1 (or just under 1).}
\ppz{For example, greedy user carbon optimization and provisioning strategies are now aligned, they both lead to preferring using older machines.}

\akj{Show how load levelization is bad in this model, if there is availability on older machines they should be heavily utilized.}
\ppz{scheduling Y, Z are not good. For example, using scheduling Z, will generate utilization of 0.3, 0.3, and 0.3 on fast, medium, and slow machines, this carbon cost is more expensive than greedy scheduling, which generates 0.9 utilization on slow machines; when using DDB, and considering the idle time. And also if we do not use DDB, we will never see the difference among these scheduling methods.}
\ppz{data here}\akj{talk about this in the traditional way, cost per job, no idle cost}

\akj{need experiment to show how workloads with different QoS constraints and greedy optimizations of carbon can benefit from this carbon modeling ($model_{dep}$), and are aligned with carbon efficient provisioning (particularly when considering idle time).}

-------- maybe we don't do this

\akj{Show how bringing onboard machines that are over-provisioned has a high penalty, because you have to pay for the idle $C_{emb}$.} \akj{cannot ignore idle cost}
\ppz{related to burstiness}

\akj{However, bringing onboard more OLD machines is much less painful, because yes there is some $C_{emb}$ but it is small.  This is how you prefer to load up newer machines if you want to do that.}

----------------

\akj{There needs to be some $C_{emb}$ added for older machines for maintenance: e.g., replacing faulty memory, SSDs, CPUs, etc.}
\akj{dont for get these commented references}


==> tables/AppParam.tex <==
\begin{table}
    \centering
    
    \caption{Details of different deep learning applications.}
    \footnotesize
    \begin{tabular}{ccc|ccc}
        \hline
        App. & Task & Param. &  App. & Task & Param.  \\
        \hline
        DenseNet & CV & 7.98M &  Bert-l & NLP & 340M\\
        \hline
        ResNet50 & CV & 25.56M &  OPT-2.7B & LLM & 2.7B\\
        \hline
         Resnet 101 & CV & 44.55M& Falcon-7B & LLM & 7B  \\
        \hline
         VGG19 & CV & 143.65M & Persimmon-8B & LLM & 8B\\
        \hline
        Bert-b & NLP & 110M &  \\
        \hline
        
    \end{tabular}
    
    \label{tbl:applicationModel}
\end{table}

% \begin{table}
%     \centering
    
%     \caption{Details of different deep learning models.}
%     \footnotesize
%     \begin{tabular}{ccc|ccc}
%         \hline
%         App. & Task & Param. &  App. & Task & Param.  \\
%         \hline
%         DenseNet & CV & 7.98M & VGG19 & CV & 143.65M \\
%         \hline
%         ResNet50 & CV & 25.56M & Bert-l & NLP & 340M \\
%         \hline
%         Resnet 50-local & CV & 25.56M & OPT-2.7B & LLM & 2.7B \\
%         \hline
%         Resnet 101 & CV & 44.55M & Falcon-7B & LLM & 7B \\
%         \hline
%         Bert-b & NLP & 110M & Persimmon-8B & LLM & 8B \\
%         \hline
        
%     \end{tabular}
    
%     \label{tbl:applicationModel}
% \end{table}
    
    


==> tables/AppParam1.tex <==
\begin{table}
    \centering
    \caption{Details of different applications.}
    \begin{tabular}{ccc|ccc}
        \hline
        App. & Task & Param. &  App. & Task & Param.  \\
        \hline
        DenseNet & CV & 7.98M & VGG19 & CV & 143.65M \\
        \hline
        ResNet50 & CV & 25.56M & Bert-l & NLP & 340M \\
        \hline
        Resnet 50-local & CV & 25.56M & OPT2.7b & LLM & 2.7B \\
        \hline
        Resnext 101 & CV & 44.55M & Falcon7b & LLM & 7B \\
        \hline
        Bert-b & NLP & 110M & Persimmon8b & LLM & 8B \\
        \hline
        
    \end{tabular}
    
    \label{tab:mytable}
\end{table}


==> tables/Modeled_individual_components.tex <==
\begin{table}
    \centering
    \centering
    \caption{Three generations of GPUs and corresponding CPUs equipped in the three generations of servers.
    %Modeled individual components.
    }
    \begin{tabular}{cccccc}
        \hline
        Type & Name & Node & Die Size & TDP & Date \\
        \hline
        \hline
        
        GPU & \makecell{NVIDIA\\ V100} & 12nm & 815$\text{mm}^2$ & 300W & 2017 \\
        \hline
        GPU & \makecell{NVIDIA\\ A10G} & 8nm & 628$\text{mm}^2$ & 300W & 2021 \\
        \hline
        GPU & \makecell{NVIDIA \\RTX5000Ada} & 5nm & 609$\text{mm}^2$ & 250W & 2023 \\
        \hline

        CPU & \makecell{Xeon E5 \\2686 v4} & 14nm & 456$\text{mm}^2$ & 145W & 2016 \\
        \hline
        CPU & \makecell{AMD \\EPYC 7R32} & 7nm & N/A & 280W & 2020 \\
        \hline
        CPU & \makecell{Intel Xeon \\Gold 6346} & 10nm & N/A & 205W & 2021 \\
        \hline
    \end{tabular}
    \label{tab:components}
\end{table}


==> tables/improvement.tex <==
\begin{table}
    \centering
    \caption{Throughput Improvement of different application groups}
    \begin{tabular}{ccccc}
        \hline
        Improvement & Overall & CV & NLP & LLM \\
        \hline
        System 1 to 2 & 1.15 & 1.32 & 0.94 & 1.11 \\
        \hline
        System 3 to 4 & 1.72 & 1.74 & 1.70 & 1.26 \\
        \hline
    \end{tabular}

    \label{improvement}
\end{table}


==> tables/server_config.tex <==
\begin{table}
\centering
\small
\caption{
Server configurations used for the carbon footprint report across vendors. A star~\mystar ~ means the configuration is ``important" in estimating the manufacturing/embodied cost.
% HP reports all the ``important" features.
}
\label{tab:config_breakdown}
\begin{adjustbox}{width=1\columnwidth,center}
\begin{tabular}{c|c|c|c|c}
\hline
&  & HP & Dell & Lenovo \\ \hline 
%\rotatebox[origin=c]{90}
\multirow{10}{*}{{Manufacturing}} & \#CPUs & \checkmark & \checkmark & \checkmark \\ %\hline
& Total CPU \#Cores~\mystar  & \checkmark & & \\ %\hline
& Memory (GB)~\mystar  & \checkmark & \checkmark & \\ %\hline
& SSD \#disks  & \checkmark & \checkmark & \checkmark \\ %\hline
& Total SSD size (GB)~\mystar  & \checkmark & & \\ %\hline
& HDD \#disks  & \checkmark & \checkmark & \checkmark \\ %\hline
%& Total HDD size~\mystar  &&& \\ %\hline
& \#Fans &&& \checkmark \\
& \#PSU & \checkmark && \\
& Server type & \checkmark & \checkmark & \checkmark \\ 
& Release year~\mystar  & \checkmark & \checkmark & \checkmark \\ \hline
\multirow{2}{*}{{Transport}} & Region & \checkmark & \checkmark & \checkmark \\
& Server Weight & \checkmark & \checkmark & \checkmark \\
& Transportation Method & && \checkmark \\ \hline
\multirow{3}{*}{{Use}} & Product Lifetime & \checkmark & \checkmark & \checkmark \\
& Yearly Energy (TEC) & \checkmark & \checkmark & \\
& TEC Configs & \checkmark && \\ \hline
EOL & EOL Methods & && \checkmark \\ \hline
\end{tabular}
%}
\end{adjustbox}
%  {\raggedright \\
%  Note: 
%  {  %\color{violet}Purple} indicates architecture and mapping framework. 
%  .
%  \par}
%  }
\end{table}

